Low-Complexity Soft-Decision Detection for Combating DFE Burst Errors in IM/DD Links

The deployment of non-binary pulse amplitude modulation (PAM) and soft decision (SD)-forward error correction (FEC) in future intensity-modulation (IM)/direct-detection (DD) links is inevitable. However, high-speed IM/DD links suffer from inter-symbol interference (ISI) due to bandwidth-limited hardware. Traditional approaches to mitigate the effects of ISI are filters and trellis-based algorithms targeting symbol-wise maximum a posteriori (MAP) detection. The former approach includes decision-feedback equalizer (DFE), and the latter includes Max-Log-MAP (MLM) and soft-output Viterbi algorithm (SOVA). Although DFE is easy to implement, it introduces error propagation. Such burst errors distort the log-likelihood ratios (LLRs) required by SD-FEC, causing performance degradation. On the other hand, MLM and SOVA provide near-optimum performance, but their complexity is very high for high-order PAM. In this paper, we consider a one-tap partial response channel model, which is relevant for high-speed IM/DD links. We propose to combine DFE with either MLM or SOVA in a low-complexity architecture. The key idea is to allow MLM or SOVA to detect only 3 typical DFE symbol errors, and use the detected error information to generate LLRs in a modified demapper. The proposed structure enables a tradeoff between complexity and performance: (i) the complexity of MLM or SOVA is reduced and (ii) the decoding penalty due to error propagation is mitigated. Compared to SOVA detection, the proposed scheme can achieve a significant complexity reduction of up to 94% for PAM-8 transmission. Simulation and experimental results show that the resulting SNR loss is roughly 0.3 to 0.4 dB for PAM-4, and becomes marginal 0.18 dB for PAM-8.

==> Algorithm_ST_Dmp.tex <==
\begin{algorithm}[t]
\KwIn{DFE-equalized symbol $\yeq_i$, DFE-3 LLR $\Gamma_i(s)$, and noise variance $\sigma^2$}
\KwOut{ Bit-wise LLRs $[L^{S}_{i,j}]$}


% \For{$i=1,2,...,N$}{
\For{$j=1,2,...,\log_2{M}$}{  
\begin{align}\label{Eq:MaxLog_State_LLR}
     L^{S}_{i,j}= & \max\limits_{s\in\mcS}  \Biggr[ \Gamma_i(s) -  \nonumber  \\
      & \left.  \left(\min\limits_{x\in\mcX_k^1}[|\yeq_i-x-h \omega(s)|]\right)^2/(2\sigma^2)  \right] \nonumber \\
      & -\max\limits_{s\in\mcS}  \Biggr[ \Gamma_i(s) -  \nonumber  \\
      & \left.  \left(\min\limits_{x\in\mcX_k^0}[|\yeq_i-x-h \omega(s)|]\right)^2/(2\sigma^2)  \right] 
 \end{align}
  

% \begin{align}
%     \tilde{p}_{B1}  = & \max \Biggr[ \tilde{p}(s_i=c,\by)-\frac{\left(\min\limits_{x\in\mcX_k^1}[|\yeq_i-x|]\right)^2}{2\sigma^2}, \nonumber \\
%     & \tilde{p}(s_i=l,\by)-\frac{\left(\min\limits_{x\in\mcX_k^1}[|\yeq_i-x+\alpha d|]\right)^2}{2\sigma^2}, \nonumber \\
%     & \tilde{p}(s_i=r,\by)-\frac{\left(\min\limits_{x\in\mcX_k^1}[|\yeq_i-x-\alpha d|]\right)^2}{2\sigma^2} \Biggr] \nonumber
% \end{align}

% \begin{align}
%     \tilde{p}_{B0}  = & \max \Biggr[ \tilde{p}(s_i=c,\by)-\frac{\left(\min\limits_{x\in\mcX_k^0}[|\yeq_i-x|]\right)^2}{2\sigma^2}, \nonumber \\
%     & \tilde{p}(s_i=l,\by)-\frac{\left(\min\limits_{x\in\mcX_k^0}[|\yeq_i-x+\alpha d|]\right)^2}{2\sigma^2}, \nonumber \\
%     & \tilde{p}(s_i=r,\by)-\frac{\left(\min\limits_{x\in\mcX_k^0}[|\yeq_i-x-\alpha d|]\right)^2}{2\sigma^2} \Biggr] \nonumber
% \end{align}

 
}
% }


\KwRet{$[L^{S}_{i,j}]$}
\caption{DFE-State Max-Log Demapper}
\label{alg:DFE_ST_Dmp}
\end{algorithm}

==> Figures/Figure_BER_8PAM.tex <==

\begin{figure}[t!]
\centering
\setkeys{Gin}{width=1\textwidth}
\resizebox{1\linewidth}{!}{\input{./Figures/BER_8PAM.tikz}} 
\caption{ PAM-8 simulation results of post-FEC BER vs. SNR.}
\label{Fig:Results_Sim_8PAM}
\end{figure}

==> Figures/Figure_Result_PAM4.tex <==

\begin{figure}[t!]
\centering
\setkeys{Gin}{width=1\textwidth}
% \resizebox{1\linewidth}{!}{\input{./Figures/combiFig_0_6.tikz}}
\resizebox{1\linewidth}{!}{\input{./Figures/combiFig_0_6_v2.tikz}}
\caption{PAM-4 simulation results of (a) Pre-FEC BER vs. SNR; (b) Pre-FEC BER vs. Post-FEC BER; (c) Post-FEC BER vs. SNR.}
\label{Fig:Results_Sim}
\end{figure}

==> Tab_Complexity.tex <==


\begin{table*}
    \centering
    \caption{Complexity Comparison of the DFE-ST-MLM and the SOVA in Number of Add, Multiply, and Compare\&Select (CS) Operations.}
    \label{Tab:Ctomplx. Comp.}
    \begin{tabular}{c c c c c c c c}
    \hline\hline
    % \textbf{Scheme} & \textbf{$+/-$} & \textbf{$\times$} & \textbf{CS} & Time Complexity \\\hline
    
    \multirow{2}{*}{\textbf{Scheme}} & \multicolumn{2}{c}{\textbf{Add}} & \multicolumn{2}{c}{\textbf{Multiply}} & \multicolumn{2}{c}{\textbf{CS}} & \multirow{2}{*}{\textbf{Time Complexity}}  \\ \cline{2-7} 
    \multirow{2}{*}{} & Number & Normalization & Number & Normalization & Number & Normalization & \multirow{2}{*}{} \\\hline
    SOVA ($\delta=10$) & 5952768 & 100\% & 150144 & 100\% & 1483776 & 100\% & $O(N_s M^2 \delta)$ \\
    MLM & 724224 & 12.17\% & 17664 & 11.76\% & 141312 & 9.52\% & $O(N_s M )$ \\ \hline
    DFE-ST-SOVA ($\delta=10$) \& Demap. & 2755584 &  46.29\% & 88320 & 58.82\% & 927360 & 62.50\% & $O(N_s N_e^2 \delta)$ \\
    DFE-ST-MLM \& Demap. & 578496 &  9.72\% & 114816 & 76.47\% & 150144 & 10.12\% & $O(N_s N_e)$ \\
    DFE-ST-FWD \& Demap. & 66240 & 1.11\% & 114816 & 76.47\%  & 97152 & 6.55\% & $O(N_s N_e)$ \\
    \hline\hline
    \end{tabular}
\end{table*}



%%%%%%%%%%% Notes
\begin{comment}
Number of symbols per frame: 8832

%% 2, 3, or 4 elements select are considered the same
%%% SOVA
SOVA (trace backlength =10):

+: 8832*4*4 (update path metrics. 16 paths) + 8832*4*4 (find the path metric differences) +  8832*4*4*10*4 (trace back add and compare to update LLR) + 8832*2 (symbol llr to bit llr,  two max substract)

x: 8832*4*4 (update path metrics. 16 paths) + 8832 (symbol llr to bit llr, scaled by snr)

CS: 8832*4 (find the minimum path metric per state, 4 elements select) + 8832*4*4*10 (trace back add and compare to update LLR, 4 elements select) +  8832 *4 (symbol llr to bit llr, 4 max)

%%% DFE, See Algorithm 1
DFE:

+: 8832

x: 0

CS: 8832 (2 elements select)

%%% MLM, See Algorithm 1
MLM:

+: 
Transition prob. gamma: 8832*(3+3/4*3+3/4*3)
Three log operations: 8832*3*3 (forward) +8832*3*3 (backward) +8832*3*3*2 (combine for APP)

x:
Transition prob. gamma: 8832

CS:
Three log operations: 8832*3*2 (forward and backward 3 elements select) + 8832*3 (combine for APP 3 elements select)

%%% MLM state demapp, See Algorithm 2
MLM Demap:

+: 8832*2*3 (two max suubstract) + 8832*2*4*2 (inside the min)

x: 8832*2*2*3 (min suqre over 2 sigma^2) 

CS: 8832*2*2 (two max. 3 elements select) + 8832*2*2 (two min. 4 elements select)

%%% BCJR MLM, See Matlab code
BCJR MLM:

+: 
Transition prob. gamma: 8832*16
Three log operations: 8832*4*4 (forward) +8832*4*4 (backward) +8832*4*4*2 (combine for APP)+ 8832*2 (symbol llr to bit llr,  two max substract)

x:
Transition prob. gamma: 8832 

CS:
Three log operations: 8832*4*2 (forward and backward 4 elements select) + 8832*4 (combine for APP 3 elements select)
+  8832 *4 (symbol llr to bit llr, 4 max)

%%% DFE ST-SOVA
DFE ST SOVA (trace backlength =10):

+: 8832*3*3 (update path metrics. 9 paths) + 8832*3*3 (find the path metric differences) +  8832*3*3*10*3 (trace back add and compare to update LLR) + 8832*2 (symbol llr to bit llr,  two max substract)

x: 8832*3*3 (update path metrics. 16 paths) + 8832 (symbol llr to bit llr, scaled by snr)

CS: 8832*3 (find the minimum path metric per state, 3 elements select) + 8832*3*3*10 (trace back add and compare to update LLR, 3 elements select) +  8832 *4 (symbol llr to bit llr, 4 max)

\end{comment}


==> Tab_Complexity_CS.tex <==

\begin{table}
    \centering
    \caption{Complexity Comparison in Compare\&Select Operations Between MLM and SOVA ($\delta=10$) when Performed on PAM-$M$ ($N_s = M$) or DFE-$3$ ($N_s = 3$) State Machine.}
    \label{Tab:Ctomplx. Comp.}
    \begin{tabular}{c | c c | c c }
    \hline\hline %\addlinespace[0.1em] 
    \multirow{2}{*}{\textbf{Scheme}} & \multicolumn{2}{c|}{\textbf{SOVA}} & \multicolumn{2}{c}{\textbf{MLM}}   \\ \cline{2-3} \cline{4-5} %\addlinespace[0.1em] 
    \multirow{2}{*}{} & Number & Norm. & Number & Norm.   \multirow{2}{*}{} \\\hline \addlinespace[0.1em]
    PAM-4 & 5864448 & 100\%  & 494592 &  100\% \\
    DFE-3 & 2676096 & 45.63\%  & 450432 &  91.07\% \\\hline
    PAM-8 & 30664704 &  100\% & 1271808 & 100\%  \\
    DFE-3 & 1937152 & 6.32\%  & 453376 &  35.65\% \\\hline \addlinespace[0.1em] 
    \textbf{Time Complexity} & \multicolumn{2}{c|}{\textbf{$O(N_s^2 \delta)$}} & \multicolumn{2}{c}{\textbf{$O(N_s)$}} \\ \addlinespace[0.1em] 
    \hline\hline
    \end{tabular}
    
\end{table}


% \begin{table*}
%     \centering
%     \caption{Complexity Comparison in Compare\&Select (CS) Operations Between MLM and SOVA ($\delta=10$) when Performed Based on PAM-$M$ ($N_s = M$) or DFE-$3$ ($N_s = 3$) State Machine.}
%     \label{Tab:Ctomplx. Comp.}
%     \begin{tabular}{c c c c c c c c}
%     \hline\hline 
%     \addlinespace[0.1em]
%     \multirow{2}{*}{\textbf{Scheme}} & \multicolumn{2}{c}{\textbf{DFE-3}} & \multicolumn{2}{c}{\textbf{PAM-4}} & \multicolumn{2}{c}{\textbf{PAM-8}} & \multirow{2}{*}{\textbf{Time Complexity}}  \\ \cline{2-7} \addlinespace[0.1em] 
%     \multirow{2}{*}{} & Number & Normalization & Number & Normalization & Number & Normalization & \multirow{2}{*}{} \\\hline \addlinespace[0.1em]
%     MLM &  & 1 &  &  &  &  & $O(N_s)$ \\
%     SOVA &  &  &  &   &  &  & $O(N_s^2 \delta)$  \\
%     \hline\hline
%     \end{tabular}
    
% \end{table*}

 

%%%%%%%%%%% Notes
\begin{comment}
Number of symbols per frame N: PAM-4:8832 PAM8: 5888

%%% PAM-M MLM, See Matlab code
PAM-M BCJR MLM:

CS: N*M*2 (forward and backward M elements select) + N*M (combine for APP M elements select) +  N * log2(M) * 2 (symbol llr to bit llr, M/2 elements select)

%%% PAM-M SOVA
SOVA (trace backlength =10):

CS: N*M (find the minimum path metric per state, M elements select) + N*M*M*10 (trace back add and compare to update LLR, M elements select) +  N * log2(M) * 2 (symbol llr to bit llr, M/2 elements select)

%%% DFE, See Algorithm 1
DFE:

CS: N (M elements select)

%%% DFE-3 MLM 
DFE-3 MLM:

CS: N*3*2 (forward and backward 3 elements select) + N*3 (combine for APP 3 elements select)


%%% DFE-3 SOVA
DFE ST SOVA (trace backlength =10):

CS: N*3 (find the minimum path metric per state, 3 elements select) + N*3*3*10 (trace back add and compare to update LLR, 3 elements select)

%%% DFE-3 state demapper 
DFE-3 State Demap:

CS: N*2*log2(M) (two max. 3 elements select) + N*2*log2(M) (two min. M/2 elements select)


\end{comment}

